FRESH: Fr\'echet Similarity with Hashing

This paper studies the $r$-range search problem for curves under the continuous Fr\'echet distance: given a dataset $S$ of $n$ polygonal curves and a threshold $r>0$, construct a data structure that, for any query curve $q$, efficiently returns all entries in $S$ with distance at most $r$ from $q$. We propose FRESH, an approximate and randomized approach for $r$-range search, that leverages on a locality sensitive hashing scheme for detecting candidate near neighbors of the query curve, and on a subsequent pruning step based on a cascade of curve simplifications. We experimentally compare \fresh to exact and deterministic solutions, and we show that high performance can be reached by suitably relaxing precision and recall.

==> theory.tex <==
In this section, we overview the collision probabilities of the LSH scheme in our paper. 
For simplicity, we assume that $d=1$, that is that all curves have vertices in the real set $\Re$.

\paragraph*{\bf LSH scheme}
The theoretical analysis in~\cite[Theorem 7]{driemel_locality-sensitive_2017} shows that, under a worst case scenario, the collision probability of two curves $p$ and $q$ under the LSH family $\mathcal{\hat G}_\delta$ satisfies
\begin{align}\label{eq:collprob1}
\Pr_{g\in \mathcal{\hat G}_\delta}\left[g(p)=g(q)\right]\geq 1-\frac{2m d_{dF}(p,q)}{\delta},
\end{align}
where $m$ is the length of longest curve.
Moreover, two curves with distance $d_{dF}(p,q)>\delta$ never collide under $\mathcal{\hat G}_\delta$, that is $\Pr_{g\in \mathcal{\hat G}_\delta}\left[g(p)=g(q)\right]=0$.
If we set the gird size to $\delta=4mr$, there is at least probability $1/2$ that two $r$-near curves collide. However, this implies a large number of collisions between curves with distances in $(r, 4mr]$.
If we set $\delta$ very close to $r$, the lower bound in Equation~\ref{eq:collprob1} quickly becomes negative: this is due to the $m$ term, which follows from an union bound on the probability $\varsigma$ that at least two vertices of a component of the optimal discrete traversal of $p$ and $q$ are not mapped on the same cell of the grid $G_\delta$  (i.e., $\varsigma$ is the probability of breaking a component with the grid). Note that $\varsigma\leq 2 d_{dF}(p,q)/\delta$ and there are at most $m$ components.

We observe that a more interesting lower bound on the collision probability follows if we assume that  each input/query curve  $p$ is given by the sum of two components $p=s+n$, where $s$ is the true signal and $n$ is noise. 
When the noise is uniformly distributed in  $[-\delta/2,\delta/2)$,  we get that the collision probability is at least 
\begin{align}\label{eq:collprob2}
\Pr_{g\in \mathcal{\hat G}_\delta,n}\left[g(p)=g(q)\right] \geq \left(\frac{1}{4}-\frac{d_{dF}(p,q)}{2\delta}\right)^m.
\end{align}
(Note that the probability is also over the random noise.)
Curves with distance $d_{dF}(p,q)>2\delta$ never collide (the constant 2 is accountable to the noise and does not appear in the bound in~\ref{eq:collprob1}).
Bound in Equation~\ref{eq:collprob2} follows from the proof of an alternative LSH scheme presented in~\cite[Theorem 9]{driemel_locality-sensitive_2017}, where a uniform noise is added to each vertex of the input and query curves.
By mimic the proof in~\cite{driemel_locality-sensitive_2017}, it is also possible to show that a similar bound holds when  the noise is a normal distribution with mean 0 and standard deviation $\BT{\delta}$. 
Although the bound in Equation~\ref{eq:collprob2} does not become negative as in Equation~\ref{eq:collprob1}, we observe that the collision probability is lower bounded by an exponential term,  even with very large values of $\delta$ (the reason being that noise and grid have the same width).

Finally, for the sake of the analysis, we assume that the aforementioned  probability $\varsigma$ of breaking a component is independent of what happen to the other components (we can thus avoid the union bound). In this case, we get
\begin{align}\label{eq:collprob3}
\Pr_{g\in \mathcal{\hat G}_\delta}\left[g(p)=g(q)\right]\geq \left(1-\frac{2 d_{dF}(p,q)}{\delta}\right)^m,
\end{align}
and curves with distance $d_{dF}(p,q)>\delta$ never collide.
In this scenario, which seems to hold in our experiments, the collision probability of near points is at least $1/e$ when $\delta \geq 2m r$.
On the other hand, if $\delta$ is close to $r$ we get the exponential dependency on $m$ as in Equation~\ref{eq:collprob2}.

Finally we observe that, by setting the number of hash tables in \fresh to $L=\BT{p_1^{-k}}$, a near neighbor of $q$ collides at least once in expectation, under $\mathcal{\hat G}^k_\delta$ (if $L=\BT{p_1^{-k}\log n}$, all near neighbor of $q$ are reported with high probability. 
This claim holds also for the scheme $\mathcal{G}^k_\delta$ which is the one adopted in \fresh, since its collision probabilities are equivalent to $\mathcal{\hat G}_\delta$, as we show below.
In the experimental section, we give evidence that much smaller values of $L$ suffice for a high recall.

\paragraph*{\bf Bounding the tensoring and hashing techniques}
The tensoring and hashing approaches can potentially change the collision probabilities given in the previous paragraph.
Indeed, the tensoring approach can decrease the collision probability of near curves and the multiply-shift  hashing  can increase the collision probability of far curves. However, as we show here, both terms are negligible. 

Consider the LSH family $\mathcal{\hat G}_\delta^k$ constructed without tensoring, and let $L=\BT{p_1^{-k}}$ be the number of hash tables.
A pair of near curves $p$ and $q$ collides in at least one of the $L$ hash tables with probability at least $1-(1-p_1^k)^L\geq 1- 1/e^{p_1^k L} >1-1/e$.
Consider now the LSH family $\mathcal{ G}_\delta^k$ constructed with tensoring.
The near pair $p$ and $q$ collides in at least one of the $L$ hash tables if  $p$ and $q$ collide in at least one of the hash functions in $\Lambda_1$ and in $\Lambda_2$ (we recall that $\Lambda_1$ and $\Lambda_2$ are two sets with $\sqrt{L}$ LSH from $\mathcal{\hat G}_\delta^{k/2}$).
Since $p$ and $q$ do not collide in $\Lambda_1$ with probability $(1-p_1^{k/2})^{\sqrt{L}}$ (similarly in $\Lambda_2$), $p$ and $q$ collide in at least one of the $L$ hash tables  with probability  at least 
$1-2(1-p_1^{k/2})^{\sqrt{L}} \geq 1 - 2/e^{p_1^{k/2}\sqrt{L}} > 1- 2/e$, which is a constant factor from the probability obtained with $\mathcal{\hat G}_\delta^k$.

Let $u$ and $v$ be the parameters used in the multiply-shift  hashing scheme $\mathcal H$~\cite{Dietzfelbinger97}. 
When using the multiply-shift  hashing family, the collision probability of two far curves  increases by an additive term $1/2^{u-v}$ with respect to $\mathcal{\hat{G}}_{\delta}^k$, due to collisions under  $\mathcal H$.
However this factor is very small,  and in our experiments where $u=64$ and $v=32$, the probability is  $2^{-32}$.
Then, even with very large datasets, we expect no more than one point with distance larger than $\delta$ in the output. 
We observe that in our extensive experimental evaluation, we have not had any collision due to the multiply-shift  hashing.

\paragraph*{\bf LSH for the continuous Fréchet distance}
The collision probabilities of the LSH scheme at the base of \fresh have been studied for the discrete Fréchet distance.
An interesting question is to bound the collision probabilities in terms of the continuous Fréchet distance.
A bound follows by the following relation between the continuous and discrete Fréchet distances of two curves $p$ and $q$ by~\cite{Eiter94}:
$$
d_F(p,q) \leq d_{dF}(p,q) \leq d_{F}(p,q) + \max\{\iota_p, \iota_q\},
$$
where $\iota_p$ denotes the length of the longest edge in $p$, that is $\iota_p=\max_{1\leq i< |p|}{\|p_i-p_{i-1}\|}$.
Therefore, if we are willing to find all curves with continuous Fréchet distance less than $r_F$ from a query $q$, we should use an LSH scheme for the discrete distance with $r=r_F+\iota$, where $\iota$ is the length of the longest edge of input and query curves.
However, our experimental analysis in Section~\ref{sec:exp} shows that this bound is,  in almost all cases, quite pessimistic and that it suffices to set  $r=r_F$ in the LSH scheme to get a recall close to 1 for the continuous case. The only exception, as we will see in Section~\ref{sec:lshclassifier}, is the wafer dataset where there is a significant difference between the continuous and discrete Fréchet distances.


